Compositional Distributional Semantics with Compact Closed Categories and Frobenius Algebras

This thesis contributes to ongoing research related to the categorical compositional model for natural language of Coecke, Sadrzadeh and Clark in three ways: Firstly, I propose a concrete instantiation of the abstract framework based on Frobenius algebras (joint work with Sadrzadeh). The theory improves shortcomings of previous proposals, extends the coverage of the language, and is supported by experimental work that improves existing results. The proposed framework describes a new class of compositional models that find intuitive interpretations for a number of linguistic phenomena. Secondly, I propose and evaluate in practice a new compositional methodology which explicitly deals with the different levels of lexical ambiguity (joint work with Pulman). A concrete algorithm is presented, based on the separation of vector disambiguation from composition in an explicit prior step. Extensive experimental work shows that the proposed methodology indeed results in more accurate composite representations for the framework of Coecke et al. in particular and every other class of compositional models in general. As a last contribution, I formalize the explicit treatment of lexical ambiguity in the context of the categorical framework by resorting to categorical quantum mechanics (joint work with Coecke). In the proposed extension, the concept of a distributional vector is replaced with that of a density matrix, which compactly represents a probability distribution over the potential different meanings of the specific word. Composition takes the form of quantum measurements, leading to interesting analogies between quantum physics and linguistics.

==> frobverbs-old.tex <==
\chapter{Building Verb Tensors using Frobenius Algebras}
\label{ch:frobverbs}

\begin{chabstract}
I begin my analysis by revising the first complete study of the categorical framework \cite{GrefenstetteThesis2013}. Firstly, I offer an intuitive interpretation of the proposed model in the context of Frobenius algebras. Then I proceed and present a number of novel models, relying again on Frobenius algebras, that extend and improve the previous work in a number of ways. After I provide a linguistic intuition of the suggested framework, I conclude the chapter by presenting a new CDM hierarchy that incorporates the newly devised class of models. Material is based on \cite{kartsaklis2014,kartsadrqpl2014,kartsaklis2012}. 
\end{chabstract}

\noindent
To a great extent, the essence of any tensor-based model lies on the functions that produce the sentences, i.e. the verbs. As we saw in \S \ref{sec:intuition}, the purpose of such a function is to take a number of inputs (vectors representing nouns or noun phrases) and transform them to a sentence. The important question of how a function of this form can be constructed can obviously find more than one answers, many of which might depend on the underlying task in hand or the available resources. A goal of this thesis, though, is to not be dependent on factors of this sort; I am interested in reasoning about natural language meaning at a generic level, with the hope that the (any) findings would have to say something more than how effective a specific CDM can be in some specific task. So let me start ``by the book'' and adopt a formal semantics perspective, where the meaning of a predicate such as a verb can be seen as the set of all elements in our universe who perform the action that the verb describes. As it will become evident, this approach leads naturally to the tensor construction method of Grefenstette and Sadrzadeh \cite{GrefenSadr1}, which will serve as a starting point for the models presented in this thesis.

\section{Verb tensors as relations}
\label{sec:tensor-rel}

Recall from the discussion in \S \ref{sec:compsem} that under an extensional perspective of semantics the meaning of an intransitive verb is the following set:

\begin{equation}
  \sem{sleep} = \{x|x \in \mathcal{U} \wedge x~\text{sleeps}\}
  \label{equ:sleep-set}
\end{equation}

\noindent where $\mathcal{U}$ denotes our universe. Note that a set such as the above is in one-to-one correspondence with a \textit{characteristic function} that maps individuals from our domain $\mathcal{U}$ to truth values; in other words, Eq. \ref{equ:sleep-set} can also be given as:

\begin{equation}
  \sem{sleep} = \{(x,t)|x \in \mathcal{U}, t=\top~\text{if}~x~\text{sleeps and}~\bot~\text{o.w.} \}
\end{equation}

I will now start transfer this setting to a vector space environment, adopting a truth-theoretic instantiation similar to the example in \S\ref{sec:intuition}. We take our sentence space $S$ to be the one-dimensional space spanned by the single vector $\ov{1}$, which represents the truth value $\top$, whereas value $\bot$ is given by vector $\ov{0}$. Furthermore, the noun space $N$ is spanned by a set of mutually orthogonal vectors $\{\ov{n_i}\}_i$ denoting individuals (John is represented by $\ov{n_1}$, Mary by $\ov{n_2}$ and so on). 
% In this setting, the entirety of our universe is a vector of ones defined as $\ov{U}=\sum_i \ov{n_i}$. Given a set of individuals $A\subseteq \mathcal{U}$, it is also possible to define a vector $\ov{a}=\sum_{\ov{n} \in A} \ov{n}$ that represents that set in a vectorial form. Naturally, the $i$th element of this vector will be 1 iff the individual who is denoted by $\ov{n_i}$ is included in the set, and 0 otherwise. 
Continuing on the intransitive verb example, consider the set $A$ of all individuals who appear at least once as a subject of a specific verb in some training corpus, and take $\chi_A$ to be the characteristic function of that set. Then, by mapping each pair $(x,t)$ of $\chi_A$ to the tensor product of the vectors denoting $x$ and $t$, we can define the meaning of the verb as below:

\begin{equation}
   \label{equ:intr1-formal}
   \ol{verb}_{IN} = \sum_{(\sem{\ov{n_i}},\sem{\ov{s_i}}) \in \chi_A} \ov{n_i}\ten \ov{s_i}
\end{equation}

\noindent with $\ov{s_i}$ to be the one-dimensional vector $\ov{1}$ if the individual $\ov{n_i}$ occurs as a subject of the intransitive verb and $\ov{0}$ otherwise. The resulting tensor lives in the tensor product space $N\ten S$, as required by the grammatical type $n^r\cdot s$ assigned to intransitive verbs. Furthermore, since our sentence space is one-dimensional, the tensor of Eq. \ref{equ:intr1-formal} is isomorphic to a vector created by summing the vectors of all individuals in set $A$:

\begin{equation}
   \label{equ:intr-formal}
   \ov{verb}_{IN} = \sum_{\sem{\ov{n_i}}\in A} \ov{n_i}
\end{equation}

Naturally, the $i$th element of this vector will be 1 if the individual who is denoted by $\ov{n_i}$ is included in the set, and 0 otherwise; furthermore, the entirety of our universe will be a vector of ones defined as $\ov{U}=\sum_i \ov{n_i}$. 

% In this setting, the entirety of our universe is a vector of ones defined as $\ov{U}=\sum_i \ov{n_i}$. Given a set of individuals $A\subseteq \mathcal{U}$, it is also possible to define a vector $\ov{a}=\sum_{\ov{n} \in A} \ov{n}$ that represents that set in a vectorial form. 





\noindent with $\ov{s_i}$ to be the one-dimensional vector $\ov{1}$ iff the individual $\ov{n_i}$ occurs as a subject of the intransitive verb and $\ov{0}$ otherwise. Assuming this latter canonical form of the verb tensor, and given that individual `Mary' is denoted by $\ov{n_2}$, we can compute the meaning of the sentence ``Mary sleeps'' as follows:

\begin{eqnarray}
  \epsilon^r_N \ten 1_S \left(\ov{n_2}\ten\sum_i(\ov{n_i}\ten\ov{s_i})\right) & = &
  \epsilon^r_N \ten 1_S \left(\sum_i \ov{n_2}\ten\ov{n_i}\ten\ov{s_i}\right) \nonumber \\
  & = & \sum_i \langle\ov{n_2}|\ov{n_i}\rangle\ov{s_i} =
  \sum_i \delta_{2i}\ov{s_i} \\
  & = & \ov{s_2} \left\{ \begin{array}{lr}\ov{1} & \text{iff}~\ov{n_2}\in S \\ \ov{0} & o.w. \end{array} \right. \nonumber
\end{eqnarray}

Note that in practice this is just the inner product of the vector of Mary with the vector representing the subset of individuals who sleep, as in Eq. \ref{equ:intr-formal}.

Let us now examine the case of a word of two arguments, such as a transitive verb. From an extensional perspective, this will be a relation of the following form:

\begin{equation}
  \label{equ:trans-formal}
  likes = \{(\ov{n_i},\ov{n_j})|\sem{\ov{n_i}}~\text{likes}~\sem{\ov{n_j}}\}
\end{equation}

In order to represent this kind of set in our vectorial setting, we first map each pair $(\ov{n_i},\ov{n_j})$ in the relation to the tensor product between the two vectors $\ov{n_i}\ten\ov{n_j}$. This will be a matrix of size $|\mathcal{U}|\times|\mathcal{U}|$ with all zeros except the element in position $(i,j)$, which will be 1. It is now straightforward to model the relation of Eq. \ref{equ:trans-formal} as the sum of all pairs, in the following manner:

\begin{equation}
  \label{equ:trans1-formal}
  \ol{verb}_{TR} = \sum_{(\ov{n_s},\ov{n_o}) \in S} \ov{n_s}\ten \ov{n_o}
\end{equation}

\noindent where $\ov{n_s}$, $\ov{n_o}$ denote individuals occurring as the subject and the object, respectively, of the specific verb. The result will be a matrix with an element in position $(i,j)$ to be 1 iff $(\ov{n_i},\ov{n_j})$ has occurred as context of the verb, and 0 otherwise. As in the one-argument case, the functorial relation with the grammatical type of the verb ($n^r\cdot s \cdot n^l$) can be retained if we replace the matrix of Eq. \ref{equ:trans1-formal} with the following isomorphic form:

\begin{equation}
   \label{equ:tran2-formal}
   \ol{verb}_{TR} = \sum_{(\ov{n_i},\ov{n_j}) \in \mathcal{U}\times\mathcal{U},\ov{s_{ij}}} \ov{n_i}\ten \ov{s_{ij}} \ten \ov{n_j}
\end{equation}

\noindent where $\ov{s_{ij}}$ is a one-dimensional vector denoting the inclusion or the absence of the corresponding pair of individuals in the relation. It is trivial to show that computing the meaning of a sentence ``$\sem{\ov{n_k}}$ likes $\sem{\ov{n_l}}$'' will always result in the corresponding $\ov{s_{kl}}$ vector, i.e. the $(i,j)$th element of the matrix in Eq. \ref{equ:trans1-formal}. 

The discussion so far suggests that the ``argument tensoring-and-summing'' process described above is a valid way for one to model the truth-theoretic nature of formal approaches in natural language semantics, when one uses a vector space setting. In the first concrete implementation of the categorical framework from Grefenstette and Sadrzadeh \cite{GrefenSadr1}, the authors suggest a generalization of this method to highly dimensional real-valued vectors. Specifically, for the case of a transitive verb they propose the creation of a matrix as follows:

\begin{equation}
\label{equ:weightrel}
 \ol{verb} = \sum\limits_{i}(\ov{subj_i}\otimes \ov{obj_i})
\end{equation}

\noindent where $\ov{subj_i}$ and $\ov{obj_i}$ are the distributional vectors of subject and object, respectively, created as described in \S\ref{sec:dissem}, and $i$ iterates over all contexts of the specific verb in the training corpus. As explained in the doctoral thesis of Grefenstette \cite{GrefenstetteThesis2013}, this process has as a result a structural mixing of the argument vectors, which reflects the extent to which each component of the subject vector is compatible with all the components of the object vector, and vice versa. 

For the purposes of this thesis, the argument summing procedure of \cite{GrefenSadr1} has many important advantages. As demonstrated above, it is obviously aligned with the formal semantics perspective, which makes perfect sense for a model that can be seen as a mathematical counterpart of this traditional view of meaning in language. Furthermore, it is generic enough not to be tied in any particular task or methodology, while at the same time its implementation and testing remains straightforward. Last, but not least, it creates \textit{reduced representations} for relational words, since in all cases the order of the produced tensor is by one lower than the order dictated by the grammatical type. This is a quite important achievement, since for tensor-based models space complexity is always an issue. If, for example, we assume verb and sentence vectors with 300 dimensions, a transitive verb (a tensor of order 3) will require 27 millions parameters, while for the case of a ditransitive verb this number is increased to 8.1 billions. Overall, I consider the argument summing procedure an interesting test-bed and an appropriate tool for demonstrating the ideas presented in this thesis.

%For a verb with $n$ arguments, this transformation will require the representation of the verb as a tensor of order $n+1$ (we need $n$ ``dimensions'' for the arguments and one for the result). We have now identified one of the most important problems of tensor-based models: in general, high-order tensors are objects hard to create and manipulate efficiently. If, for example, we assume verb and sentence vectors with 300 dimensions, a transitive verb (a tensor of order 3) will require 27 millions parameters, while for the case of a ditransitive verb this number is increased to 8.1 billions. Furthermore, it is not uncommon for functional words such as prepositions and relative pronouns to require tensors of order 5 or even 6, depending on their usage. This shows that the elegant mathematical formulations on paper are not directly applicable in practical situations. Part of this thesis aims to address this problem by creating and using reduced tensor representations in a canonical way, consistent with the theoretical basis. I will start working towards this end from the next section, reviewing and extending a specific implementation proposal. 

%\section{A first attempt for simplification}
%\label{sec:relational}
%
%The first concrete implementation of the categorical framework for simple transitive sentences comes from Grefenstette and Sadrzadeh \cite{GrefenSadr1}, and is described in detail in the doctoral thesis of first author \cite{GrefenstetteThesis2013}. In this work, the authors argue that the distributional meaning of a relational word is the sum of its arguments. An adjective, for example, is represented as the sum of all vectors of the nouns that this adjective modifies in the training corpus. Similarly, a relational word with two arguments, such as a transitive verb, is initially represented as a matrix created by structurally mixing and summing up all the contexts (subject and object pairs) in which the verb occurs, as follows:
%
%\begin{equation}
%\label{equ:weightrel}
% \ol{verb} = \sum\limits_{i}(\ov{subj_i}\otimes \ov{obj_i})
%\end{equation}
%
%\noindent where $\ov{subj_i}$ and $\ov{obj_i}$ are the context vectors of subject and object, respectively, and $i$ iterates over all contexts of the specific verb. Regarding our discussion in the introduction of this chapter, this method has the advantage that it creates a \textit{reduced representation} for the relational word; indeed, in all cases the order of the produced tensor is by one lower than the order dictated by the grammatical type. 
%
%In \cite{GrefenSadr1} and \cite{GrefenstetteThesis2013}, the meaning of a sentence is represented as an order-$n$ tensor, where $n$ is the number of arguments for the head word of the sentence. In other words, an intransitive sentence lives in a space $S=N$, a transitive one in $S=N\otimes N$ and so on. As the authors show by following the linear-algebraic calculations, this design decision leads to the following formula for representing the meaning of a transitive sentence:
%
%\begin{equation}
%  \ol{s_{TR}} = \ol{verb} \odot (\ov{subj} \ten \ov{obj})
%  \label{equ:reltrans}
%\end{equation}
% 
%The reduced tensor representations produced by Eq. \ref{equ:weightrel} have two important advantages: first, they offer an intuitive extensional notion of meaning, very much aligned with the formal semantics perspective; second, their implementation and testing is straightforward. Overall, they constitute interesting objects, and for this reason they will serve as a starting point and a useful test-bed for the research presented in this thesis. 

% Note that at this point the functorial relation of \textbf{FVect} with the pregroup grammar has been lost; in a certain sense, restoring properly this relation is the subject of the rest of this chapter.

% The reduced tensor representations of \cite{GrefenSadr1} will serve as the starting point of the research presented in this thesis. 

%In \cite{GrefenSadr1} and \cite{GrefenstetteThesis2013}, the meaning of a sentence is represented as an order-$n$ tensor, where $n$ is the number of arguments for the head word of the sentence. In other words, an intransitive sentence lives in a space $S=N$, a transitive one in $S=N\otimes N$ and so on. For the transitive case, this design decision leads to the following computation for representing the meaning of a sentence:
%
%\begin{equation}
%  \ol{s_{TR}} = \ol{verb} \odot (\ov{subj} \ten \ov{obj})
%  \label{equ:reltrans}
%\end{equation}
%
%In order to fit this to the categorical framework, an explicit function is utilized of the following form  \cite{GrefenstetteThesis2013}:
%
%\begin{equation}
%  f^{\textit{verb}}: N \ten N \to N \ten N:: \ov{subj} \ten \ov{obj} \mapsto \overline{verb} \odot (\ov{subj} \ten \ov{obj}) 
%  \label{equ:reled}
%\end{equation}
%
%This function was directly applied on the inputs of the verb (subject/object pair), transforming the categorical composition\footnote{The term \textit{categorical composition} in this text refers to composition according to the categorical framework of Chapter \ref{ch:framework}, unless stated otherwise.} to the form presented in Fig. \ref{fig:reled}.
%
%\begin{figure}[h!]
%\footnotesize
%\ctikzfig{edrel}
%\normalsize
%\caption{Composition using an explicit function.}
%\label{fig:reled}
%\end{figure}

\section{Introducing Frobenius algebras in language}
\label{sec:recast}

\tikzstyle{every picture}=[scale=0.35,baseline=0pt]

Despite the many benefits of the reduced tensors presented in \S\ref{sec:tensor-rel}, there is still an important problem we have to solve in order to make this method viable for real-world tasks. Recall that in its current form, our sentence space is one-dimensional. The transition from the truth-theoretic setting to real-valued vector spaces means that the single element that will result in from a composition would not be restricted to 0 or 1, but it would be some number that, under proper normalization conditions, can show how much \textit{probable} is the specific subject-object pair for the verb at hand. Our composition function in this case is nothing more than an endomorphism of the field:

\begin{equation}
  I \cong I\ten I \ten I \xrightarrow{\ov{s}\ten\ol{v}\ten\ov{o}}N\ten N \ten N \ten N \xrightarrow{\epsilon^r_N \ten \epsilon^l_N} I\ten I \cong I
\end{equation}

For any practical application, this is of course inadequate. We need a way to \textit{physically} expand the verb matrix into a tensor of higher order, thus providing somehow the sentence dimension that is now missing. Remember from our discussion in \S \ref{sec:frobenius} that every vector space with a fixed basis has a Frobenius algebra over it, which provides canonical ways for \textit{copying} or \textit{deleting} elements of that basis. Since in this case we are interested in copying, our tool will be a Frobenius map $\Delta: N \to N\ten N$, applied on one or more of the original dimensions of our matrix, which currently lives in $N\ten N$. 

As it turns out, the decision of which (and how many) dimensions of the verb matrix to copy has some important consequences. We will start by examining the case of copying both dimensions, in which our inflated tensor takes the following form:

\begin{equation}
  I \xrightarrow{\ol{verb}} N\ten N \xrightarrow{\Delta_N \ten \Delta_N} N\ten N \ten N \ten N
\end{equation}

How does this tensor form fits to the grammatical type $n^r\cdot s \cdot n^l$? What we implicitly assume here is that $S=N\ten N$, which means that the composition of a transitive verb with a specific subject-object pair will result in a matrix. In fact, this is exactly the composition model proposed in \cite{GrefenSadr1} and \cite{GrefenstetteThesis2013}, where the meaning of a sentence is represented as an order-$n$ tensor, with $n$ to be the number of arguments for the head word of the sentence. In other words, when following this approach an intransitive sentence lives in a space $S=N$, a transitive one in $S=N\otimes N$ and so on. Let us show this graphically; in our diagrammatic calculus, the inflated tensor is depicted by the left-hand diagram below. When substituting the verb in Def. \ref{def:categorical}, the composition proceeds as in the right-hand diagram:

\begin{equation}
\footnotesize
\tikzfig{rel} 
\normalsize
\label{fig:frobrel-ed}
\end{equation}
\vspace{0.3cm}

It is immediately obvious that the involvement of $\Delta$-maps in the creation of the verb tensor imposes a restriction: since now our sentence space is produced by copying basis elements of the noun space, our functor $\mathcal{F}$ cannot any more apply different mappings on the two atomic pregroup types $\{s,n\}$; both of these should be mapped onto the same basic vector space, bringing the model closer to vector mixtures than originally indented by the theory. 

Indeed, it is easy to show that in the extreme case that one copies \textit{all} the dimensions of a relational tensor, as we do here, the model reduces itself to a simple point-wise multiplication of the arguments with the verb tensor itself. This is exactly what diagram (\ref{fig:frobrel-ed}) reflects, and it is also obvious from the closed-form formula produced by the composition: Let $\ov{subj} = \sum_i s_i \ov{n_i}$, $\ov{obj} = \sum_j o_j \ov{n_j}$ be the vectors for the context of a transitive verb, the initial matrix of which is given by $\ol{verb} = \sum_{ij} v_{ij} \ov{n_i} \ten \ov{n_j}$. Then, let $\ol{verb}~' = \Delta_N\ten \Delta_N(\ol{verb})=\sum_{ij} v_{ij} \ov{n_i} \ten \ov{n_i} \ten \ov{n_j} \ten \ov{n_j}$; the categorical composition proceeds as follows:

   \begin{eqnarray}
     \epsilon^r_N \ten 1_{N\ten N} \ten \epsilon^l_N
     (\ov{subj} \ten \ol{verb}~' \ten \ov{obj}) & = \nonumber \\
     \sum\limits_{ij} v_{ij} \langle \ov{subj}|\ov{n_i} \rangle \langle \ov{n_j}|\ov{obj} \rangle \ov{n_i} \ten \ov{n_j} & = \\
     \sum\limits_{ij} v_{ij} s_i o_{j} \ov{n_i} \ten \ov{n_j} = \ol{verb} \odot (\ov{subj} \ten \ov{obj}) \nonumber
   \end{eqnarray}

Hence, what we actually get is a sophisticated version of a vector mixture model, where the representation of a sentence is always \textit{the tensor product of the arguments scaled by the tensor of the head verb} (see discussion in \S \ref{sec:intuition}). Which now makes very clear the reason behind a second unwelcome property of this formulation, that every sentence has to live in a space of a different tensor power, equal to that of the head verb. Especially this latter side-effect is in direct conflict with the premises of the categorical framework, since there is no way for one to compare sentences of different structures, say an intransitive one with a transitive one. Even more importantly, it means that the model is unable to assign a meaning to sentences or phrases with nested grammatical structures, such as in the following case:

\begin{equation}
\small
\tikzfig{mary}
\normalsize
\end{equation}

Due to the mismatch between the logical and the concrete types, the translation of the above derivation to vector spaces is not possible; the linear map for `read' expects a vector in $N$ as a semantic representation for its subject, but what actually receives is a tensor of order 2 (a matrix). The next section deals with all the above issues.


%In \cite{GrefenSadr1} and \cite{GrefenstetteThesis2013}, the meaning of a sentence is represented as an order-$n$ tensor, where $n$ is the number of arguments for the head word of the sentence. In other words, an intransitive sentence lives in a space $S=N$, a transitive one in $S=N\otimes N$ and so on. As the authors show by following the linear-algebraic calculations, this design decision leads to the following formula for representing the meaning of a transitive sentence:
%
%\begin{equation}
%  \ol{s_{TR}} = \ol{verb} \odot (\ov{subj} \ten \ov{obj})
%  \label{equ:reltrans}
%\end{equation}
% 
%
%The decision of taking $S=N\ten N$ has some interesting consequences for the form of the verb tensor. Starting from the pregroup type of a transitive verb ($n^r\cdot s \cdot n^l$) we get:
%
%\begin{equation}
%  \mathcal{F}(n^r\cdot s \cdot n^l) = N \ten S \ten N = N \ten N \ten N \ten N
%\end{equation}
%
%Therefore, in order for the model to be consistent with the theoretical basis, the initial verb matrix needs to be \textit{expanded} (somehow) to a tensor of order 4. Remember from our discussion in \S \ref{sec:frobenius} that every vector space with a fixed basis has a Frobenius algebra over it, which provides canonical ways for \textit{copying} or \textit{deleting} elements of that basis. I will now proceed to show that Eq. \ref{equ:reltrans} is nothing more than a closed-form formula for categorical composition\footnote{The term \textit{categorical composition} in this text refers to composition according to the categorical framework of Chapter \ref{ch:framework}, unless stated otherwise.} after the application of Frobenius $\delta$ maps on both dimensions of the verb matrix.
%
%\begin{proposition}
%\label{prop:relfrob}
%  Eq. \ref{equ:reltrans} is equivalent to standard categorical composition applied on $1_N\ten \delta_N\ten \delta_N\ten 1_N (\ov{subj} \ten \ol{verb} \ten \ov{obj})$.
%\end{proposition}
%
%\begin{proof}
%   Let $\ov{subj} = \sum_i s_i \ov{n_i}$, $\ov{obj} = \sum_j o_j \ov{n_j}$ be the vectors for the context of a transitive verb, the initial matrix of which is given by $\ol{verb} = \sum_{ij} v_{ij} \ov{n_i} \ten \ov{n_j}$. Then, let $\ol{verb}~' = \delta_N\ten \delta_N(\ol{verb})=\sum_{ij} v_{ij} \ov{n_i} \ten \ov{n_i} \ten \ov{n_j} \ten \ov{n_j}$, and the categorical composition proceeds as follows:
%   \begin{eqnarray*}
%     \epsilon^r_N \ten 1_{N\ten N} \ten \epsilon^l_N
%     (\ov{subj} \ten \ol{verb}~' \ten \ov{obj}) & = \\
%     \sum\limits_{ij} v_{ij} \langle \ov{subj}|\ov{n_i} \rangle \langle \ov{n_j}|\ov{obj} \rangle \ov{n_i} \ten \ov{n_j} & = \\
%     \sum\limits_{ij} v_{ij} s_i o_{j} \ov{n_i} \ten \ov{n_j} = \ol{verb} \odot (\ov{subj} \ten \ov{obj})
%   \end{eqnarray*}
%\end{proof}
%
%In our diagrammatic calculus, the inflated tensor is depicted as shown by the left-hand diagram below. When substituting the verb in Def. \ref{def:categorical}, the composition proceeds as in the right-hand diagram:
%
%\begin{equation}
%\footnotesize
%\tikzfig{rel} 
%\normalsize
%\label{fig:frobrel}
%\end{equation}
%
%\vspace{0.5cm}
%%The complete transformation of the pregroup type to a tensor now takes the following, more aligned to the theoretical basis, form:
%%
%%\begin{equation}
%%  n^r\cdot s \cdot n^l\xrightarrow{\mathcal{~F~}} N \ten N \ten N \xrightarrow{1_N \ten \delta_N \ten 1_N} N \ten N \ten N \ten N
%%  \label{equ:expand}
%%\end{equation}
%
%The involvement of the Frobenius $\delta$-map in the creation of the verb tensor imposes an unwelcome restriction: since now our sentence space is produced by copying basis elements of the noun space, our functor $\mathcal{F}$ cannot any more apply different mappings on the two atomic pregroup types $\{s,n\}$; both of these should be now mapped onto the same basic vector space, bringing the model closer to vector mixtures than originally indented by the theory. 
%
%Indeed, it is easy to show that in the extreme case that one copies \textit{all} the dimensions of a relational tensor, as we do here, the model reduces itself to a simple point-wise multiplication of the arguments with the verb tensor itself. This is exactly what Eq. \ref{equ:reltrans} and diagram (\ref{fig:frobrel}) reflects. Hence, what we actually get is a sophisticated version of a vector mixture model, where the representation of a sentence is always \textit{the tensor product of the arguments scaled by the tensor of the head verb} (see discussion in \S \ref{sec:intuition}). Which now makes very clear the reason behind a second unwelcome property of this formulation, that every sentence has to live in a space of a different tensor power, equal to that of the head verb. Especially this latter side-effect is in direct conflict with the premises of the categorical framework, since there is no way for one to compare sentences of different structures, say an intransitive one with a transitive one. The next section deals with all the above issues.


\section{Unifying the sentence space}
\label{sec:sentencespace}

The remedy for the issues raised with the approach of \cite{GrefenSadr1} is simple and comes directly from the two main rules we are required to follow: (a) $S$ must be equal to $N$; (b) a tensor with $n$ arguments will always return a vector in $N$ iff its order is $n+1$. Since we start from reduced tensors, the order of which is equal to the number of the verb arguments, this simply means that in order to properly restore the functorial passage from grammar to vector spaces we have to restrict ourselves in copying only \textit{one} of the tensor dimensions. As we will see later, this leads to interesting consequences that allow intuitive linguistic interpretations of the framework. 

I will continue using the case of a transitive verb as a running example. We start from a matrix created as dictated by Eq. \ref{equ:weightrel}. This is a tensor living in $N \ten N$ that has to be encoded in $N \ten N \ten N$. A transitive verb is a function of two arguments, so there are two different ways to apply the Frobenius $\Delta$-map:

\paragraph{Copy-Subject} The first option is to copy the ``row'' dimension of the linear map corresponding to the verb. This dimension is the one that interacts with the subject noun during the composition. In diagrammatic form, the tensor and the composition are as follows:

\begin{equation}
\footnotesize
\tikzfig{copysbj} 
\label{fig:copysbj}
\end{equation}

\vspace{0.5cm}
The compositional morphism in this case is the following:

\begin{eqnarray}
  (\epsilon^r_N \ten 1_N \ten \epsilon^l_N) \circ 
  (1_N \ten \Delta_N \ten 1_N \ten 1_N)
  (\ov{subj} \ten \ol{verb} \ten \ov{obj}) & = \\
  \mu_N\ten\epsilon^l_N(\ov{subj} \ten \ol{verb} \ten \ov{obj}) 
  \nonumber
 \label{equ:csbj-cat}
\end{eqnarray}

\noindent as the normal form in (\ref{fig:copysbj}) and the diagram below makes clear:

\begin{equation}
\begin{tikzpicture}[scale=1.5,baseline=30pt]
font=\footnotesize
\node (A) at (0,4) {$I\ten I\ten I$};
\node (B) at (8,4) {$N\ten N\ten N\ten N$};
\node (C) at (20,4) {$N\ten N\ten N\ten N\ten N$};
\node (D) at (20,0) {$N$};
\path[->,font=\scriptsize]
(A) edge node[above]{$\ov{s}\ten\ol{v}\ten\ov{o}$} (B)
(B) edge node[above]{$1_N\ten \Delta_N \ten 1_N\ten 1_N$} (C)
(C) edge node[left]{$\epsilon^r_N\ten 1_N \ten \epsilon^l_N$} (D)
(B) edge node[left]{$\mu_N \ten \epsilon^l_N~~~~$} (D);
\end{tikzpicture}
\end{equation}

Linear-algebraically (and using the subject, verb, and object vectors of our previous example), the computation proceeds as follows:

\begin{eqnarray}
\mu_N\ten\epsilon_N^l(\ov{subj}\ten\ol{verb}\ten\ov{obj}) =
\sum\limits_{ij}v_{ij}s_io_j \mu_N(\ov{n_i}\ten\ov{n_i}) \epsilon^l_N(\ov{n_j}\ten \ov{n_j}) & = \nonumber \\
\sum\limits_{ij}v_{ij}s_io_j \ov{n_i} \langle \ov{n_j}|\ov{n_j} \rangle = \sum\limits_{ij}v_{ij}s_io_j \ov{n_i} & = \\
\ov{subj} \odot (\ol{verb} \times \ov{obj}) \nonumber
\end{eqnarray}

\paragraph{Copy-Object} Our other option is to copy the ``column'' dimension of the verb matrix, the one that interacts with objects:

\begin{equation}
\footnotesize
\tikzfig{copyobj} 
\label{fig:copyobj}
\end{equation}

\vspace{0.5cm}
Eq. \ref{equ:cobj-cat} provides the categorical morphism, while the linear algebraic form (which I am not going to derive explicitly this time) is shown in Eq. \ref{equ:cobj-lalg}.

\begin{eqnarray}
  \label{equ:cobj-cat}
  (\epsilon^r_N \ten 1_N \ten \epsilon^l_N)\circ
  (1_N\ten 1_N\ten \delta_N \ten 1_N) 
  (\ov{subj} \ten \ol{verb} \ten \ov{obj}) & = \\
  \epsilon^r_N \ten \mu_N
  (\ov{subj} \ten \ol{verb} \ten \ov{obj}) \nonumber
\end{eqnarray}
\vspace{-0.6cm}
\begin{equation}
   \ov{s_{TR}} = \ov{obj} \odot (\ol{verb}^{\mathsf{T}} \times \ov{subj})
  \label{equ:cobj-lalg}
\end{equation}

From a geometric perspective, the two Frobenius models correspond to different ways of ``diagonally'' placing a plane into a cube. This is shown in Fig. \ref{fig:cubes}.

\begin{figure}[h!]
  \footnotesize
  \ctikzfig{cubes}
  \normalsize
  \caption{Geometric interpretation of the Frobenius models.}
  \label{fig:cubes}
\end{figure}

On the contrary with the original model of \cite{GrefenSadr1}, the interpretation of the Copy-Subject and Copy-Object models is quite different. Although there is still an element of point-wise multiplication, now part of the sentence is computed by tensor contraction. For the case of the Copy-Subject model, this part is the verb phrase (verb-object) which is produced by matrix-multiplying the verb matrix with the object vector. In other words, what actually it is achieved is a merging of the vector of the subject with the composite vector of the verb phrase.

\begin{equation}
 \footnotesize
 \tikzfig{copysbj-normal}
 \normalsize
\end{equation}

\vspace{0.5cm}
The situation is very similar for the Copy-Object model, with the difference that now a vector is ``categorically'' composed for the intransitive part of the sentence (subject-verb), and then this vector is merged with the vector of the object:

\begin{equation}
 \footnotesize
 \tikzfig{copyobj-normal}
 \normalsize
\end{equation}

\vspace{0.5cm}
The particular perspective of breaking the sentence into two parts with the verb as a common joint provides another important advantage: it actually \textit{justifies} the somewhat ad-hoc decision to use a matrix in the compositional equations, since in both the cases of a verb phrase and an intransitive sentence the verb is a function of a single argument---that is, it can be canonically represented as a tensor of order 2. Actually, my analysis suggests that the matrix in the Copy-Subject model must be different from the matrix of the Copy-Object model, since these two tensors actually represent different functions. I will return to this topic in \S \ref{sec:frob-regression}, when I will discuss statistical techniques for building the relational tensors. For now, I will show how the Frobenius setting can be extended to tensors of any arity.

\section{Extending the setting to any tensor}
\label{sec:ditransitive}

The application of Frobenius operators extends to any relational word, providing a generic treatment for all aspects of language.   According to the ``argument summing'' procedure of \cite{GrefenSadr1}, for example, the linear maps of adjectives and intransitive verbs (both functions of a  single argument) will be elements of $N$ created as follows:

\begin{equation}
   \ov{adj} = \sum\limits_i \ov{noun_i}\quad\quad\quad
   \ov{verb}_{IN} = \sum\limits_i \ov{subj_i}
\end{equation}

\noindent with $i$ iterating through all relevant contexts. In both cases the application of a $\Delta$ operation will create a diagonal matrix, which when substituted in Def. \ref{def:categorical} will produce the result shown below. 

\begin{equation}
\footnotesize
\tikzfig{adj-intr}
\normalsize
\label{fig:single-arg}
\end{equation}

This is another case of copying ``all'' dimensions of a tensor (here just one), that as we discussed in \S \ref{sec:sentencespace} results in a degeneration to an element-wise multiplicative model. Specifically, the meaning of adjective-noun compounds and intransitive sentences reduces to the following:

\vspace{-0.5cm}
\begin{gather}
  \ov{adj~noun} = \mu(\ov{adj}\ten\ov{noun}) = \ov{adj} \odot \ov{noun} \\
  \ov{s_{IN}} = \mu(\ov{subj}\ten\ov{verb}) = \ov{subj} \odot \ov{verb} 
\end{gather}

I will now proceed to the more interesting case of a ditransitive sentence, the derivation of which is depicted here: 

\begin{equation}
%\begin{center}
\begin{minipage}{0.35\linewidth}
  \footnotesize
  \ctikzfig{dtrans-preg}
\end{minipage}
\begin{minipage}{0.35\linewidth}
   \footnotesize
   \ctikzfig{dtrans}
\end{minipage}
%\end{center}
%\caption{Categorical composition for ditransitive verbs.}
\label{fig:dtrans}
\end{equation}

A ditransitive verb can be seen as a function of 3 arguments; hence, we can start by creating a tensor of order 3 that represents the verb, as follows:

\begin{equation}
  \ol{verb}_{DT} = \sum\limits_i \ov{subj_i} \ten \ov{iobj_i} \ten \ov{dobj_i}
\end{equation}

\noindent
where $\ov{iobj}$ and $\ov{dobj}$ refer to the vectors of the indirect and direct object, respectively. In this case, the Frobenius operators offer to us three alternatives, all of which are shown below:

\begin{eqnarray}
  %\begin{center}
  \begin{minipage}{0.35\linewidth}
    \footnotesize
    \ctikzfig{dt-copysbj}
    \centering
    Copy subject
  \end{minipage}
  \begin{minipage}{0.35\linewidth}
    \footnotesize
    \ctikzfig{dt-copydobj}
    \centering
    Copy direct object
  \end{minipage} \\\nonumber
  ~\\\nonumber
  \begin{minipage}{0.70\linewidth}
    \footnotesize
    \ctikzfig{dt-copyiobj}
    \centering
    Copy indirect object
  \end{minipage}
  \label{fig:frob-ditrans}
\end{eqnarray}

\vspace{0.2cm}
Note that in all cases the result is a vector, computed as below:

\begin{equation}
  \text{Copy subject:}~\ov{s_{DT}} = \ov{subj} \odot \left((\ol{verb} \times \ov{iobj})\times \ov{dobj} \right)
  \label{equ:copysbj-dit}
\end{equation}

\vspace{-0.6cm}
\begin{equation}
  \text{Copy direct object:}~\ov{s_{DT}} = \ov{dobj} \odot \left((\ol{verb}\times \ov{iobj})^{\mathsf{T}} \times \ov{subj} \right)
  \label{equ:copydobj-dit}
\end{equation}

\vspace{-0.6cm}
\begin{equation}
  \text{Copy indirect object:}~\ov{s_{DT}} = \ov{iobj} \odot \left((\ol{verb}\times \ov{dobj})^{\mathsf{T}} \times \ov{subj} \right)
  \label{equ:copyiobj-dit}
\end{equation}

As in the transitive case, the sentence is broken into two parts: one part for the copied argument and one part for the rest of the sentence. In all cases, the argument vector is scaled by point-wise multiplication with the composite vector of the context. Let me now formally define the concept of a \textit{Frobenius  vector} as follows:

\begin{definition}
\label{def:frobvector}
  Let a text constituent with head word $w$ of arity $n$ and grammatical derivation $\alpha$; the $i$th Frobenius vector of this constituent is defined as follows:
  
  \begin{equation}
    \ov{v}_i^{\mathsf{F}} = \mathcal{F}(\alpha) (\ov{arg_1}\ten \hdots \ten \Delta_i(\ol{w}) \ten \hdots \ten \ov{arg_n})
  \end{equation}
  
\noindent where $\Delta_i(\ol{w})$ represent the application of a Frobenius $\Delta$-map on the $i$th dimension of $\ol{w}$ for brevity.

\end{definition}

%\begin{definition}
%  The \textit{Frobenius vector set} of a text constituent with head word $w$ of arity $n$ is the set of all its Frobenius vectors:
%  
%  \begin{equation}
%     S^{\mathsf{F}}_w = \{\ov{v}^{\mathsf{F}}_i | 1 \leq i \leq n \}
%  \end{equation}
%\end{definition}

If $w$ is a verb, then the Frobenius vectors $\ov{v}^{\mathsf{F}}_i$ will represent different aspects of the meaning of a sentence. In the next section I will provide an intuitive interpretation of these different aspects in the context of intonation.

\section{Modelling intonation}
\label{sec:intonation}

The term \textit{intonation} refers to variations of spoken pitch, the purpose of which is to emphasize parts of the utterance that might be important for the conveyed message. Consider again the ditransitive sentence of \S \ref{sec:ditransitive}:

\begin{exe}
\ex\label{ex:john} John gave Mary a flower
\end{exe}

This statement might have been used in response to a number of questions, each one of which requires the use of a different intonation pattern from the speaker. For example:

\begin{exe}
  \ex
  \begin{xlist}
  \ex \textit{Who did give Mary a flower?}\\
      \textbf{\underline{John}} gave Mary a flower
  \ex \textit{What did John give to Mary?}\\
      John gave Mary \textbf{\underline{a flower}}
  \ex \textit{To whom did John give a flower?} \\
      John gave \textbf{\underline{Mary}} a flower    
  \end{xlist}    
\end{exe}

The bold-faced part above is what Steedman \cite{steedman2000information} calls \textit{rheme}---the information that the speaker wishes to make common ground for the listener. The rest of the sentence, i.e. what the listener already knows, is called \textit{theme}. In the same paper, Steedman argues that the different syntactic derivations that one can get even for very simple sentences when using Combinatory Categorical Grammar (CCG) \cite{steedman} (referred to with the somewhat belittling term ``spurious readings''), actually serve to reflect changes in the intonational patterns. In CCG, our example sentence in (\ref{ex:john}) has a number of different syntactic derivations, two of them are the following:

\begin{equation}
\begin{minipage}{0.80\linewidth}
\begin{center}  
\deriv{4}{
{\rm John} & {\rm gave} & {\rm Mary} & {\rm a~flower} \\
\uline{1} & \uline{1} &\uline{1} & \uline{1} \\
NP & ((S\bs NP)/NP)/NP & NP & NP \\
   & \fapply{2} & \\
   & \cmc{2}{(S\bs NP)/NP} & \\
   & \fapply{3} \\
   & \cmc{3}{S\bs NP} \\
\bapply{4} \\
\cmc{4}{S} \\
}  
\end{center}
\end{minipage}
\label{fig:spur1}
\end{equation}

\begin{equation}
\begin{minipage}{0.80\linewidth}
\begin{center}  
\deriv{4}{
{\rm John} & {\rm gave} & {\rm Mary} & {\rm a~flower} \\
\uline{1} & \uline{1} &\uline{1} & \uline{1} \\
NP & ((S\bs NP)/NP)/NP & NP & NP \\
\ftype{1} & \fapply{2} & \\
{S/(S\bs NP)} & \cmc{2}{(S\bs NP)/NP} & \\
\fcomp{2} & & \\
\cmc{3}{S/NP} & \\
\fapply{4} \\
\cmc{4}{S} \\
}  
\end{center}
\end{minipage}
\label{fig:spur2}
\end{equation}

Note that (\ref{fig:spur1}) proceeds by first composing the part of the verb phrase (``gave Mary a flower''); later, in the final step, the verb phrase is composed with the subject `John'. The situation is reversed for (\ref{fig:spur2}), where the use of type-raising and composition rules of CCG allow the construction of the fragment ``John gave Mary'' as valid grammatical text constituent, which is later combined with the direct object of the sentence (`a flower'). According to Steedman, each one of these derivations expresses a different intonational pattern, distinguishing the rheme from the theme when the sentence is used for answering different questions:  (\ref{fig:spur1}) answers to ``Who did give Mary a flower?'', whereas (\ref{fig:spur2}) to ``What did John give to Mary?''. 

It is interesting to note that in our grammatical formalism, pregroup grammars, variations in a grammatical derivation similar to above are only implicitly assumed, since the order of composition between a relational word and its argument remains unspecified. This fact is apparent in the pregroup derivation of our sentence in (\ref{fig:dtrans}), and is directly reflected in our semantic space through the functorial passage:

\begin{eqnarray}
  \nonumber
 \ov{john}^{\mathsf{T}} \times  \left( (\ol{gave} \times \ov{mary}) \times \ov{flower} \right) & = \\
  \left( (\ov{john}^{\mathsf{T}} \times \ol{gave}) \times \ov{mary} \right) \times \ov{flower} & = \\
  \left( (\ov{john}^{\mathsf{T}} \times \ol{gave})^{\mathsf{T}} \times \ov{flower} \right) \times \ov{mary} \nonumber
\end{eqnarray}

However, if the claim that different grammatical derivations (thus different ways of combining constituents) subsume different intonational patterns is true, then this must also be reflected somehow in the semantic form of the sentence; in our case, the sentence vector. In other words, the claim here is that the meaning of sentence ``\textbf{\underline{Mary}} wrote a book about bats'' is slightly different of that of sentence ``Mary wrote a book about \textbf{\underline{bats}}''. Indeed, if one uses the former form instead of the latter to answer the question ``I \textit{know} that Mary wrote a book, but what was this book about?'', the person who posed the question will require a moment of mental processing to translate the semantics of the response in her mind.

The Frobenius setting detailed in this chapter provides a natural way to incorporate this kind of slight variations in the meaning of sentences. Recall that each one of the alternative options for copying a dimension of a tensor results in (a) splitting the sentence in two parts, one of which consists of a single argument and one for the rest of the sentence; (b) composing a vector for the rest of the sentence; and (c) point-wise multiplying the vector of the argument with the composite vector. I argue that the isolated argument corresponds to the rheme, while the composite part serves as the theme. The point-wise multiplication of the two parts provides a unified meaning for the sentence, in which however the rheme will play a very important role: the nature of the compositional operator (a vector mixture) guarantees that the resulting vector will be affected \textit{equally} from both arguments, rheme and theme. This puts the necessary focus on the appropriate part of the sentence, reflecting the variation in semantics intended by the intonational pattern:

\begin{exe}
\ex
\begin{xlist}
 \ex Who did give Mary a flower?\\
     $\ov{john} \odot \ov{gave~mary~a~flower}$
 \ex What did John give to Mary?\\
     $\ov{john~gave~mary} \odot \ov{a~flower}$
 \ex To whom did John give a flower?\\
     $\ov{john~gave~a~flower} \odot \ov{(to)~mary}$
\end{xlist} 
\end{exe}

\begin{definition}
  The meaning of a text constituent with head word $w$ and arity $n$ carrying intonational information on the $i$th argument is given by its $i$th Frobenius vector.
\end{definition}

There is a different kind of question that has not been addressed yet:

\begin{exe}
\ex What just happened?\\
    \textbf{\underline{John gave Mary a flower}}
\end{exe}

For simple declarative cases such that the above, where the theme is unmarked, it makes sense to define the meaning of a sentence as the sum of all intonational patterns. Since each intonational pattern corresponds to a different Frobenius vector, as these defined in Def. \ref{def:frobvector}, we conclude to the following:

\begin{definition}
\label{def:frobadd}
  The meaning of a sentence with an unmarked theme is defined as the sum of all its Frobenius vectors:
  
  \begin{equation}
     \ov{s_U} = \ov{v}^{\mathsf{F}}_1 + \ov{v}^{\mathsf{F}}_2 \hdots + \ov{v}^{\mathsf{F}}_n
  \end{equation}
\end{definition}

The model of Def. \ref{def:frobadd} (to which I will refer as \textbf{Frobenius additive}) can be seen as providing the meaning of a generic declarative sentence, and its effectiveness will be evaluated in Chapter \ref{ch:frobexp}. 
%since it will comprise the basis for a number of models in Chapter \ref{ch:regression}, where the tensors of relational words are learned through statistical learning (specifically linear regression). 
For now, I will provide a theoretical example of the Frobenius setting that hopefully will make the concept better understood to the reader.

%For now, I will proceed to a generic algorithm for computing the meaning of a sentence using the convenient ``argument summing'' procedure of \cite{GrefenSadr1}.

\section{A truth-theoretic instantiation}
\label{sec:truth-theoretic}

In this section, I will show how the Frobenius framework behaves in a truth-theoretic setting similar to that of \S\ref{sec:tensor-rel}. Recall that a relation corresponding to the meaning of a transitive verb, such as `likes', can be given by a matrix $\ol{likes}=\sum likes_{ij} \ov{n_i}\ten\ov{n_j}$ where $likes_{ij}$ is the scalar 1 if $\sem{\ov{n_i}}$ likes $\sem{\ov{n_j}}$ and 0 otherwise. For individuals denoted by $\ov{n_1}$ and $\ov{n_3}$, copying the subject dimension of this matrix proceeds as follows:

\begin{eqnarray}
\label{equ:likes-frob}
\mu_N \ten \epsilon^l_N \left( \ov{n_1} \ten \left( \sum\limits_{ij} likes_{ij} \ov{n_i} \ten \ov{n_j}\right) \ten \ov{n_3} \right) & = \nonumber \\
%\mu_N \ten \epsilon^l_N \left( \sum\limits_{ij} likes_{ij} \ov{n_1} \ten \ov{n_i} \ten \ov{n_j} \ten \ov{n_3} \right) & = \\
\sum\limits_{ij} likes_{ij} \mu(\ov{n_1}\ten \ov{n_i}) \langle \ov{n_j}|\ov{n_3} \rangle = 
\sum\limits_{ij} likes_{ij} \delta_{1i} \delta_{j3} \ov{n_i} & = \\ likes_{13} \ov{n_1} = 
\left\{ \begin{array}{lr} \ov{n_1} & \text{if~}likes_{13}=1 \\ \ov{0} & o.w. \end{array} \right. \nonumber
\end{eqnarray}

The above example illustrates clearly the necessity of a shared space between sentences and words when using Frobenius operators. However, how one can interpret the result of (\ref{equ:likes-frob}) in a way consistent with the model? Let us repeat the derivation step-wise, starting from the composition of the verb with the object:

\begin{eqnarray}
  1_N \ten \epsilon^l_N \left( \left( \sum\limits_{ij} likes_{ij} \ov{n_i}\ten \ov{n_j} \right) \ten \ov{n_3} \right) =
  \sum\limits_{ij} likes_{ij} \ov{n_i} \langle \ov{n_j}|\ov{n_3}\rangle & = \\
  \sum\limits_{ij} likes_{ij} \ov{n_i} \delta_{j3} = \sum\limits_{i} likes_{i3} \ov{n_i} \nonumber
\end{eqnarray}

The vectorial representation of the verb phrase ``likes $\sem{\ov{n_3}}$'' gets a very intuitive explanation: it is the sum of all individuals who like the individual denoted by vector $\ov{n_3}$. Since in our setting individuals form an orthonormal basis, the $i$th element of this vector corresponds to the individual denoted by $\ov{n_i}$, and has value 1 if this individual likes $\sem{\ov{n_3}}$ or 0 otherwise. Indeed, as we discussed in \S\ref{sec:tensor-rel} this sum can be seen as a \textit{subset} of elements in our universe, the entirety of which is represented by the vector $\sum_i \ov{n_i}$. 

What differentiates the Frobenius setting from the standard categorical composition is the second step, in our case that of composing the meaning of the verb phrase with the subject. Recall that this is just the point-wise multiplication of the vector of the verb phrase with the vector of the subject, which in our setting can be interpreted as the \textit{intersection} of the singleton set formed by the subject with the set of people who like individual $\sem{\ov{n_3}}$. 

\begin{equation}
  \ov{n_1} \odot \ov{likes~n_3} = 
  \left( \begin{array}{c} 0\\1\\0\\0 \end{array} \right) \odot
  \left( \begin{array}{c} 1\\1\\0\\1 \end{array} \right) = 
  \left( \begin{array}{c} 0\\1\\0\\0 \end{array} \right)
\end{equation}

This is just a test of set membership: if the result is the subject vector, this means that the corresponding individual is a member of the people who like $\sem{\ov{n_3}}$; in the opposite case, the result will be the zero vector (the empty set). Let us summarize these observations using as an example the concrete sentence ``John likes Mary''. In the traditional categorical composition, the meaning of this sentence is given by:

\begin{equation}
  \text{John}~\in~\{x|x~\text{likes Mary}\}
\end{equation}

\noindent and the result can be one of the two values in our sentence space, i.e. $\top$ or $\bot$. In the Frobenius setting, the meaning of the sentence changes to:

\begin{equation}
   \{\text{John}\} \cap \{x|x~\text{likes Mary}\}
\end{equation}

\noindent and the result is $\{\text{John}\}$ if John is among the people who like Mary, or the empty set otherwise. Hence, while the goal is still the same (to state the truth or falseness of the sentence), now we have a different way to express the result.

The above analysis provides a direct justification of why the Frobenius models constitute an appropriate way of modelling intonation: when answering the question ``Who likes Mary?'', the correct answer is ``John'' and not ``true'' or ``false''. Note that under this interpretation, the empty set simply represents ``nobody''. Furthermore, it is not difficult to show that when the object dimension of the verb matrix is copied, the evaluation of the sentence takes the following form:

\begin{equation}
   \{\text{Mary}\} \cap \{x|x~\text{is liked by John}\}
\end{equation}

A positive result ($\{\text{Mary}\}$) answers directly to the question ``Whom John likes?'', setting the focus on the appropriate part of the sentence. 

%\section{A generic algorithm}
%\label{sec:algorithm}
%
%\section{Encoding non-predicative models}
%
%It is interesting to see how the framework introduced in \S \ref{sec:recast} and \S \ref{sec:sentencespace} can actually accommodate simpler non-predicative models, essentially encoding them to follow categorical composition. For example, to represent the model of \cite{Lapata} in our setting (Eq. \ref{equ:mult}), in which the meaning of a sentence is simply the point-wise multiplication of the context vectors of the words, we need to apply the following morphism to the context vector of the verb:
%
%\begin{equation}
%  (1_N \ten \mu_{N\ten N} 1_N) \circ (\delta_N \ten \delta_N) \circ \delta_N
%\end{equation}
%
%\noindent
%and then proceed to categorical composition as usual. Diagrammatically, we give to the verb the form depicted in the left-hand part of (\ref{fig:frob-mult}); composition then proceeds as in right-hand part. Note that the normal form of the diagram corresponds to a simple point-wise multiplication of the three context vectors, as required by the model.
%
%\begin{equation}
%  \footnotesize
%  \tikzfig{frobmult}
%  \normalsize
%  \label{fig:frob-mult}
%\end{equation}
%\vspace{0.3cm}

\section{Frobenius operators and entanglement}
\label{sec:entanglement}

In this section I will shortly demonstrate the benefits of using Frobenius operators for constructing relational tensors with regard to \textit{entanglement}. As in quantum mechanics, entanglement is a necessary requirement for tensor-based models to allow the unhindered flow of information between the different parts of the sentence. Recall that a word tensor living in vector space $W$ is seen as a state of $W$. This state is \textit{separable} if it can be expressed as the tensor product of two vectors. In our graphical calculus, these objects  are depicted  by  the juxtaposition of two or more triangles:

\begin{equation}
\footnotesize
\tikzfig{separ}
\normalsize
\end{equation}

In general, a state is not separable if it is a linear combination of many separable states. The number of separable states needed to express the original tensor is equal to  the \textit{tensor rank}. Graphically, a tensor of this form is shown as a single triangle with two or more legs: 

\begin{equation}
\footnotesize
\tikzfig{entang}
\normalsize
\end{equation}

In categorical quantum mechanics terms, entangled states are necessary to allow the flow of information between the different subsystems; this is exactly the case for linguistics as well. Consider the diagram below, in which all relational words are represented by separable tensors (in other words, no entanglement is present). 

\begin{equation}
\label{equ:degrade}
\footnotesize
\tikzfig{sentencesep}
\normalsize
\end{equation}

In this version, the  $\epsilon$-maps are  completely detached from the components of the relational tensors that carry the results (left-hand wire of the adjective and middle wire of the verb); as a consequence, flow of information is obstructed, all compositional interactions have been eliminated, and the meaning of the sentence is reduced to the middle component of the verb (shaded vector) multiplied by a scalar, as follows (superscripts denote the left-hand, middle, and right-hand components of separable tensors):

\begin{equation*}
  \langle \ov{happy}^{(r)}|\ov{kids}\rangle \langle \ov{happy}^{(l)}|\ov{play}^{(l)} \rangle 
  \langle \ov{play}^{(r)}|\ov{games}\rangle \ov{play}^{(m)} 
\end{equation*}

Depending on how one measures the distance between two sentences, this is a very unwelcome effect, to say the least. When using cosine distance, the meaning of all sentences with `play' as the verb will be exactly the same and equal to the middle component of the  `play' tensor. For example, the sentence  ``trembling  shadows play hide-and-seek'' will have the same meaning  as our example sentence. Similarly, the comparison of two arbitrary transitive sentences will be reduced to comparing just the middle components of their verb tensors, completely ignoring any surrounding context. The use of Euclidean distance instead of cosine would slightly improve things, since now we would be at least able to also detect differences in the magnitude between the two middle components. Unfortunately, this metric has been proved not very appropriate for distributional models of meaning, since in the vastness of a highly dimensional space every point ends up to be almost equidistant from all the others. As a result, most implementations of distributional models prefer the more relaxed metric of cosine distance which is length-invariant. Table \ref{tbl:cons} presents the consequences of separability in a number of grammatical constructs.

\renewcommand{\arraystretch}{2.0}% Wider
\begin{table}[h!]
  \begin{center}
  \scriptsize
  \begin{tabular}{l|l|c}
     \hline
     \textbf{Structure} & \textbf{Simplification} & \textbf{Cos-measured} \\
     \hline\hline
      adjective-noun & $\overline{adj} \times \ov{noun} = (\ov{adj}^{(l)} \otimes \ov{adj}^{(r)}) \times \ov{noun} = \langle \ov{adj}^{(r)}|\ov{noun}\rangle \cdot \ov{adj}^{(l)}$ & $\ov{adj}^{(l)}$  \\
      \hline
     intrans. sentence & $\ov{subj} \times \overline{verb} = \ov{subj} \times (\ov{verb}^{(l)} \otimes \ov{verb}^{(r)}) = \langle \ov{subj}|\ov{verb}^{(l)}\rangle \cdot \ov{verb}^{(r)}$ & $\ov{verb}^{(r)}$  \\
     \hline
     verb-object & $\overline{verb} \times \ov{obj} = (\ov{verb}^{(l)} \otimes \ov{verb}^{(r)}) \times \ov{obj} = \langle \ov{verb}^{(r)}|\ov{obj}\rangle \cdot \ov{verb}^{(l)}$ &  $\ov{verb}^{(l)}$ \\
     \hline
     transitive sentence & $\begin{array}{r l} \ov{subj} \times \overline{verb} \times \ov{obj} =  
            \ov{subj} \times (\ov{verb}^{(l)} \otimes \ov{verb}^{(m)} \otimes \ov{verb}^{(r)}) \times \ov{obj} & = \\ 
            \langle \ov{subj}|\ov{verb}^{(l)}\rangle \cdot \langle \ov{verb}^{(r)}|\ov{obj}\rangle \cdot \ov{verb}^{(m)} \end{array}$ &  $\ov{verb}^{(m)}$\\
     \hline
  \end{tabular}
  \normalsize
  \end{center}

  \caption[Consequences of separability in various grammatical structures.]{Consequences of separability in various grammatical structures. Superscripts $(l)$, $(m)$ and $(r)$ refer to left-hand, middle, and right-hand component of a separable tensor}
  \label{tbl:cons}
\end{table}
  \renewcommand{\arraystretch}{1.0}% Wider
  
This aspect of tensor-based models of meaning is quite important and, surprisingly, almost completely neglected by the current research.  In fact, the only relevant work I am aware of comes from personal research (joint with Sadrzadeh) \cite{kartsadrqpl2014}. In the context of current discussion, the interesting point is that no matter what the actual entanglement level of relational tensors is, the Frobenius framework detailed in this chapter provides an additional layer that avoids the degrade of the composition to the ``constant'' vectors showed in (\ref{equ:degrade}). More specifically, when one copies both dimensions of the original verb matrix the result is the following:

\begin{equation}
\tikzfig{relsep}
\end{equation}

\noindent which means that, linear-algebraically, the meaning of a transitive sentence takes this form:

\begin{equation}
 \ol{subj~verb~obj} = (\ov{subj} \odot \ov{verb}^{(l)}) \otimes (\ov{verb}^{(r)} \odot \ov{obj})
\end{equation} 

Furthermore, the Copy-Subject and Copy-Object models simplify to the following:

\begin{equation}
\begin{tabular}{ccc}
 \tikzfig{copysbjsep} & & \tikzfig{copyobjsep}
\end{tabular}
\end{equation}

Therefore, the actual equation behind the Frobenius additive model is:

\begin{equation}
\ov{subj~verb~obj} = (\ov{subj} \odot \ov{verb}^{(l)}) + (\ov{verb}^{(r)} \odot \ov{obj})
  \label{equ:frobadd}
\end{equation}

Despite the simplifications presented above, note that none of these models degenerates to the level of producing ``constant'' vectors or matrices. The reason behind this lies in the use of Frobenius $\Delta$ operators for copying the original dimensions of the verb matrix, a computation that equips the fragmented system with flow, although not in the originally intended sense. The compositional structure is still fragmented into two parts, but at least now the copied dimensions provide a means to deliver the results of the two individual computations that take place, one for the left-hand part of the sentence and one for the right-hand part. I refer the interested reader to \cite{kartsadrqpl2014} for more details about this topic.

\section{From argument summing to linear regression}
\label{sec:frob-regression}

Most of my analysis in this chapter assumes as a starting point the reduced verb representations produced by applying Eq. \ref{equ:weightrel}. I will now explore a different approach based on statistical learning that, as we are going to see, fits quite nicely to the Frobenius setting, and even extends its power. Recall that the Frobenius model essentially acts on two steps: (a) it prepares a composite vector for the theme by applying tensor contraction; and (b) point-wise multiples the result with the rheme. When the rheme is the subject of a transitive verb, this is translated to the following:

\begin{equation}
 \label{equ:reg-copysbj}
 \ov{subj}\odot(\ol{verb}\times\ov{obj})
\end{equation}

\noindent with the meaning of the verb-object part to be computed ``categorically'', as the matrix multiplication of the verb with the object vector. 

Let me now attempt for a moment a twist of perspective, and forget any assumptions about using Frobenius operators. How one can describe the compositional model depicted in Eq. \ref{equ:reg-copysbj} in that case? Well, this is obviously a vector mixture model, where the operands are always some rheme and its corresponding theme; furthermore, the vector of the theme has been prepared ``categorically''. However, there is an important difference between this new view and the Frobenius one we were discussing so far: note that now the notion of a well-defined sentence does not exist any more---actually, it has to be replaced by the notion of a \textit{well-defined theme}. Let us  formalize this, by replacing type $s$ with a new atomic type, call it $\theta$. The pregroup derivation for the theme part of Eq. \ref{equ:reg-copysbj} becomes:

\begin{equation}
  (\theta\cdot n^l) \cdot n = \theta\cdot (n^l \cdot n)  \to \theta
  \label{equ:preg-theme}
\end{equation}

The new view reveals two important things. First, it is now evident why the representation of the verb as a tensor of order 2 (a matrix) makes sense in this setting: it is just a function that inputs a noun and outputs a well-defined theme, that is, $\ol{verb}:N \to \Theta$, which can canonically be expressed as a matrix in $N\ten \Theta\cong N\ten N$. More importantly, computing the meaning of the theme resulting in by copying the object dimension, in $(\ov{subj}^{\mathsf{T}} \times \ol{verb}) \odot \ov{obj}$, will naturally require a different version of $\ol{verb}$, since this time the output of our function is a syntactically different construct (subject-verb).

Assuming now we have a means to prepare these two different aspects of our verb tensor, we can think of a transitive verb as been represented by a tuple $(\ol{verb}_s,\ol{verb}_o)$. This form has the advantage that, while it retains the benefits of our previous reduced representation (we still do not need to create a verb tensor of order 3), it is more expressive since the interaction of the verb with each argument is handled by a specialized function. Using this in our Frobenius additive model results in the following equation:

\begin{equation}
  \ov{subj~verb~obj} = \ov{subj}\odot (\ol{verb}_o\times \ov{obj}) + (\ov{subj}^{\mathsf{T}}\times \ol{verb}_s)\odot \ov{obj}
  \label{equ:fadd-regr}
\end{equation}

At this stage, the separation of a transitive sentence into two distinct themes by the Frobenius operators makes easier for us to apply more sophisticated statistical methods in order to create the corresponding verb tensors. Imagine for example the case of the left-hand theme (subject-verb); what we want is a linear map $\ol{verb}_s$ that, given an input noun, will approximate some ideal distributional behaviour of the subject-verb construct in a large corpus. Assuming that, for the $i$th occurrence of the verb in the corpus, this ``ideal behaviour'' is denoted by a vector $\ov{subj_i~verb}$, with $subj_i$ referring to the corresponding subject noun, the matrix we seek is the following:

\begin{equation}
   \hat{\ol{verb}_s} = \underset{\textbf{W}}{\arg\min} \sum\limits_i \left( \textbf{W} \times \ov{subj_i} - \ov{subj_i~verb} \right)^2
   \label{equ:linregr}
\end{equation}

Learning the matrix $\textbf{W}$ that minimizes the sum in Eq. \ref{equ:linregr} is a \textit{multi-linear regression} problem, a technique that obviously constitutes the most appropriate way for training a model based on linear and multi-linear maps. What remains to be answered is how one should create the vectors that will be used as a ``gold reference'' in the optimization process. In one of the first applications of linear regression for CDMs, Baroni and Zamparelli \cite{Baroni} propose the creation of a distributional vector for every two-word construct using the same techniques as for single words (i.e. by collecting word co-occurrences from the context). The goal of the model, then, would be to create a matrix that when multiplied with a subject vector will approximate the corresponding co-occurrence vector of the subject-verb construct. Of course, exactly the same method can be applied on the right-hand theme of a transitive sentence, learning a verb matrix that produces as output a verb-object construct.

Interestingly, if we discard the point-wise multiplications in Eq. \ref{equ:fadd-regr}, what we get back is very close to a recent trend in constructing tensor-based compositional models where each argument of a multi-linear map is addressed separately by learning a specialized matrix \cite{paperno2014,polajnar2014}. These models follow a methodology very similar to what described in this section, in the sense that the composition function does not aim to produce a sentence, but a specific part of it; after that, the individual parts are somehow combined (usually by summing their vectors) to produce a vectorial representation for the whole sentence.

The decoupling of the arguments in the above way hides an important caveat: although the objective function of Eq. \ref{equ:fadd-regr} guarantees that the result will be a reliable (to the extent that the training corpus allows) map which, given an input, will produce an appropriate meaning vector for the left-hand (or right-hand) part of the sentence, there is no any guarantee whatsoever that the addition of these two vectors reflects appropriately the meaning of the whole sentence. The solution to this problem is to restore our initial perspective and start again working with sentences instead of themes. From a statistical point of view, the proper way to do that is to \textit{jointly} learn the two matrices of a transitive verb; in the case of the Frobenius additive model, this could be done by training a regression model that minimizes the following quantity:

\begin{equation}
   \sum\limits_i \left( (\textbf{W_s} \times \ov{subj_i}) \odot \ov{obj_i} + (\textbf{W_o} \times \ov{obj_i}) \odot \ov{subj_i} - \ov{subj_i~verb~obj_i} \right)^2
   \label{equ:lr-fradd}
\end{equation}

\noindent or, for the simpler version without the point-wise interaction:

\begin{equation}
   \sum\limits_i \left( \textbf{W_s} \times \ov{subj_i} + \textbf{W_o} \times \ov{obj_i} - \ov{subj_i~verb~obj_i} \right)^2
   \label{equ:lr-fradd-sim}
\end{equation}

In the above equations, $\ov{subj~verb~obj}$ refers to a distributional vector created from the contexts of the specific triplet across the corpus. Inevitably, this might lead to data sparsity problems when creating the vectors for the triplets, and certainly is not applicable for training argument matrices in cases of relational words of higher arity (e.g. ditranstive verbs). For these cases, we have to adopt the less generic solution to optimize the objective function directly on the goal set by the underlying task---for example, on some form of classification as in the case of sentiment analysis. 
%DK: Perhaps I should add an equation for the order-3 case here?

The application of the linear regression method can be seen in practice in \S\ref{sec:wsdfull}, where I use Eq. \ref{equ:linregr} in order to train matrices for verbs taking one argument.

\section{A revised taxonomy of CDMs}
\label{sec:rev-taxonomy}

The Frobenius framework presented in this chapter has the unique characteristic that it allows the combination of two quite different compositional models: a vector mixture model based on point-wise multiplication, where both operands have equal contribution to the final composite result; and a tensor-based model where relational words are tensors of higher order acting on vectors. As we saw in the previous pages, this flexibility can be used to provide solutions with intuitive linguistic interpretations, as in the case of intonation and entanglement. In Chapter \ref{ch:extend} I move one step further, showing that appropriate use of Frobenius operators can help us to reduce the space complexity imposed by the higher order tensors of functional words such as prepositions and conjunctions in a way that makes linguistic sense. 

In general, the application of Frobenius algebras to language constitutes an interesting novel compositional methodology, resulting in a class of CDMs that deserves its own place in the taxonomy we put together in Fig. \ref{fig:taxonomy}. I will now call this class \textit{partial tensor-based models}\footnote{Thanks to a suggestion by Mehrnoosh Sadrzadeh.}, and I will introduce it in Fig. \ref{fig:rev-taxonomy} below.

\begin{figure}[h!]
  \includegraphics[scale=0.86]{./pdfpic/hierarchy-rev}
  \caption{A revised taxonomy of CDMs.}
  \label{fig:rev-taxonomy}
\end{figure}
